Walking without a Map: Optimizing Response Times of Traversal-Based Linked Data Queries (Extended Version)

The emergence of Linked Data on the WWW has spawned research interest in an online execution of declarative queries over this data. A particularly interesting approach is traversal-based query execution which fetches data by traversing data links and, thus, is able to make use of up-to-date data from initially unknown data sources. The downside of this approach is the delay before the query engine completes a query execution. In this paper, we address this problem by proposing an approach to return as many elements of the result set as soon as possible. The basis of this approach is a traversal strategy that aims to fetch result-relevant data as early as possible. The challenge for such a strategy is that the query engine does not know a priori which of the data sources that will be discovered during the query execution contain result-relevant data. We introduce 16 different traversal approaches and experimentally study their impact on response times. Our experiments show that some of the approaches can achieve significant improvements over the baseline of looking up URIs on a first-come, first-served basis. Additionally, we verify the importance of these approaches by showing that typical query optimization techniques that focus solely on the process of constructing the query result cannot have any significant impact on the response times of traversal-based query executions.

==> charts_PrimaryMeasurements_W-62-47-0.tex <==
\begin{figure*}[t]
\centering
	\subfigure[\small Query Q1]{%
		\includegraphics[width=0.33\textwidth]{charts/W-62-47-0-Q1}%
		\label{sfig:PrimaryMeasurements:Q1}
	}%
	\subfigure[\small Query Q2]{%
		\includegraphics[width=0.33\textwidth]{charts/W-62-47-0-Q2}%
		\label{sfig:PrimaryMeasurements:Q2}
	}%
	\subfigure[\small Query Q3]{%
		\includegraphics[width=0.33\textwidth]{charts/W-62-47-0-Q3}
		\label{sfig:PrimaryMeasurements:Q3}
	}

	\subfigure[\small Query Q4]{%
		\includegraphics[width=0.33\textwidth]{charts/W-62-47-0-Q4}%
		\label{sfig:PrimaryMeasurements:Q4}
	}%
	\subfigure[\small Query Q5]{%
		\includegraphics[width=0.33\textwidth]{charts/W-62-47-0-Q5}%
		\label{sfig:PrimaryMeasurements:Q5}
	}%
	\subfigure[\small Query Q6]{%
		\includegraphics[width=0.33\textwidth]{charts/W-62-47-0-Q6}%
		\label{sfig:PrimaryMeasurements:Q6}
	}

	\caption{Relative response times
		%for queries Q1 to Q6 over test Web $\symWoD_\mathsf{test}^{62,47}$\!.}
		achieved by different approaches to prioritize URI lookups (test Web: $\symWoD_\mathsf{test}^{62,47}$).}
	\label{fig:PrimaryMeasurements}
\end{figure*}

==> charts_RoutingPolicies_W-62-47-0.tex <==
\begin{figure*}[t]
\centering
	\subfigure[\small Query Q3]{%
		\includegraphics[width=0.33\textwidth]{charts/W-62-47-0-Q3rpol}%
		\label{sfig:RoutingPolicies:Q1}
	}%
	\subfigure[\small Query Q4]{%
		\includegraphics[width=0.33\textwidth]{charts/W-62-47-0-Q4rpol}%
		\label{sfig:RoutingPolicies:Q4}
	}%
	\subfigure[\small Query Q6]{%
		\includegraphics[width=0.33\textwidth]{charts/W-62-47-0-Q6rpol}
		\label{sfig:RoutingPolicies:Q6}
	}

	\caption{Relative response times achieved by \is\ and \isDecr\ with different routing policies (test Web: $\symWoD_\mathsf{test}^{62,47}$).}
	\label{fig:RoutingPolicies}
\end{figure*}

==> tab_W-62-47-0.tex <==
\scriptsize
\centering
%
\begin{tabular}{|c||c|c|c|c||c|c|c|c|c||c|c|c||c|} \hline
	\cellcolor{gray!50} &
	\multicolumn{4}{c||}{\cellcolor{gray!50}link graph of reachable subweb} &
	\multicolumn{5}{c||}{\cellcolor{gray!50}result-relevant reachable documents} &
	\multicolumn{3}{c||}{\cellcolor{gray!50}res.-irrel.~reachable documents} &
	\cellcolor{gray!50}result
\\ %\hline
	\cellcolor{gray!50}Query &
	\cellcolor{gray!50}\# of &
	\cellcolor{gray!50}\# of &
	\cellcolor{gray!50}str.~connected &
	\cellcolor{gray!50}dia- &
	\cellcolor{gray!50}\# of &
	\cellcolor{gray!50}\% of all &
	\multicolumn{3}{c||}{\cellcolor{gray!50}shortest paths from seed docs} &
	\multicolumn{3}{c||}{\cellcolor{gray!50}shortest paths from seed docs} &
	\cellcolor{gray!50}cardi-
\\ %\hline
	\cellcolor{gray!50} &
	\cellcolor{gray!50}docs &
	\cellcolor{gray!50}edges &
	\cellcolor{gray!50}components &
	\cellcolor{gray!50}meter &
	\cellcolor{gray!50}docs &
	\cellcolor{gray!50}reach.docs &
	\cellcolor{gray!50}mean (st.dev) &
	\cellcolor{gray!50}min &
	\cellcolor{gray!50}max &
	\cellcolor{gray!50}mean (st.dev) &
	\cellcolor{gray!50}min &
	\cellcolor{gray!50}max &
	\cellcolor{gray!50}nality
\\ \hline
Q1	&	3834	&	10017	&	412	&	6	&	573	&	14.9\%	&	1.11		($\pm$0.43)	&	1	&	3	&	1.70		($\pm$0.93)	&	1	&	3	&	2393	\\
Q2	&	215	&	639	&	11	&	10	&	19	&	8.8\%	&	1.92		($\pm$0.58)	&	1	&	4	&	3.98		($\pm$0.91)	&	2	&	6	&	78	\\
Q3	&	168	&	290	&	46	&	6	&	5	&	3.0\%	&	1.86		($\pm$0.71)	&	1	&	3	&	2.73		($\pm$0.53)	&	1	&	3	&	6	\\
Q4	&	1097	&	7864	&	25	&	20	&	46	&	4.2\%	&	1.35		($\pm$0.72)	&	1	&	3	&	4.20		($\pm$1.04)	&	1	&	7	&	390	\\
Q5	&	333	&	2369	&	8	&	12	&	37	&	11.1\%	&	2.16		($\pm$0.72)	&	1	&	4	&	3.82		($\pm$0.37)	&	3	&	4	&	61	\\
Q6	&	2230	&	6458	&	97	&	37	&	12	&	0.5\%	&	2.26		($\pm$0.64)	&	1	&	3	&	3.97		($\pm$1.34)	&	1	&	10	&	36	\\
 \hline
\end{tabular}

==> www.tex <==
\section{Importance of Response Time Optimization} \label{sec:WWWExperiment}
\todo{...}

\smallskip\noindent
\textbf{Hypothesis:} \emph{Query execution costs are dominated by data retrieval.} (even if we use multiple threads, etc)

\smallskip\noindent
\todo{verify the hypothesis by WWW-based experiments --- for each FedBench query:}
\begin{itemize}
	\item measure the execution time, $qet$, when executed with the system described in Section~\ref{sec:Architecture}
	\item measure the execution time, $qet'$, when executed with an adjusted system whose ``data retrieval'' operator is equipped with a pre-populated cache of all reachable documents (i.e., all data is already local and nothing needs to be retrieved from the WWW)
	\item Then, $qet'$ is an approximation of the fraction of the query execution time $qet$ that has been spent on query-local processing, and $qet - qet'$ is an approximation of the fraction of query execution time spent on data retrieval
	\item expected result of this comparison: $qet' <\!< qet$
\end{itemize}
Repeat the same for different number of data retrieval threads (5, 10, 15, 20)

\bigskip\noindent
Takeaway of this exercise:
\begin{itemize}
	\item The effect of anything that can be gained by optimizing the query-local processing is marginalized by the data retrieval portion of query execution costs.
	\item Hence, query optimization should focus on data retrieval.
	\item However, no matter what source ranking strategy is applied, the same number of documents need to be retrieved for completing the query execution (with a query result that is guaranteed to be complete).
	\item Hence, the objective should be to optimize for response time (instead of overall query execution time).
\end{itemize}

